Pinned Boundaries Delay Contraction and Shape Stress Relaxation in Active Gels

Cells dynamically generate, transmit, and dissipate stress. Central to these processes is the actomyosin cortex, an active contractile material that drives cellular mechanical behavior. While prior studies have focused on freely contracting actomyosin systems, the role of mechanical constraints such as adhesion to boundaries remains less explored. To address this, we employ reconstituted actomyosin gels to investigate cellular contractility. We study contraction dynamics under pinned boundary conditions, where the gel is adhered transversely to two opposing surfaces, mimicking supracellular actomyosin networks in tissues and embryos. We find that pinned contraction leads to stress buildup, delaying contraction, producing intermittent dynamics, and generating spatially nonuniform strain fields. Stress is relieved through several pathways, including active-stress-driven symmetric constriction and defect-driven processes such as boundary detachment and internal rupture. We develop a hydrodynamic model incorporating elastic, viscous, and active stress contributions that distinguishes between stress-accumulation and stress-release phases and links variations in active stress to the observed intermittent dynamics. The model predicts distinct energy relaxation rates before and after detachment events, providing insight into stress dissipation. We compare experiments with numerical simulations, which reproduce the observed behavior and reveal how internal energy is generated and dissipated during stress buildup and relaxation. Together, our results demonstrate how boundary conditions and spatial heterogeneity govern the mechanical behavior of contractile active gels. These findings provide insight into stress regulation in cellular and tissue-scale systems and may inform the design of adaptive soft materials and bioinspired robotic systems.

==> resources/macros.tex <==
% macros - added by James Clarke 20231018

%%%%%%%%%%%
% Needed for figures
%%%%%%%%%%%
\usepackage{epsf}

%%%%%%%%%
% Needed for lists
%%%%%%%%%
\usepackage{enumitem}

% %%%%%%%%%
% % Customize fonts
% %%%%%%%%%
% \usepackage[varg]{txfonts}
% \newcommand {\bepsilon}{\mbox{\boldmath$\epsilon$}}


%%%%%%%%%%%%%
% Define custom symbols
%%%%%%%%%%%%%
\newcommand {\ltapp}   {\stackrel {_{\normalsize<}}{_{\normalsize \sim}}}
\newcommand {\gtapp}   {\stackrel {_{\normalsize>}}{_{\normalsize \sim}}}
\newcommand {\brho}    {\mbox{\boldmath$\rho$}}
\newcommand {\bbeta}   {\mbox{\boldmath$\beta$}}
\newcommand {\btau}    {\mbox{\boldmath$\tau$}}
\newcommand {\bsigma}  {\mbox{\boldmath$\sigma$}}
\newcommand {\bft}[1]   {{\textbf #1}}
%\newcommand {\em}[1]    {{\emph{#1}}}

% DEFINE HELPFUL SYMBOL SHORTCUTS
\newcommand{\inv}{^{-1}}
\newcommand{\limit}[2]{\ensuremath{\lim_{#1}{#2}}}
\newcommand{\nlog}[1]{\ensuremath{\naturallogarithm{#1}}}
%% ARROWS
% \to already exists
\newcommand{\too}[1][]{\ensuremath{\overset{#1}{\longrightarrow}}}
\newcommand{\ot}{\ensuremath{\leftarrow}}
\newcommand{\oot}[1][]{\ensuremath{\overset{#1}{\longleftarrow}}}

\newcommand{\eq}[2]{\begin{equation}{#1}\label{#2}\end{equation}}
\newcommand{\beq}[2]{\begin{equation}{\boxed{#1}\,.}\label{#2}\end{equation}}
\newcommand{\eqs}[1]{\begin{equation*}{#1}\end{equation*}}
\newcommand{\aligneq}[2]{\begin{align}{#1}\label{#2}\end{align}}
\newcommand{\aligneqs}[1]{\begin{align*}{#1}\end{align*}}
\newcommand{\m}[1]{${#1}$}
\newcommand{\fig}[3]{
	\begin{figure}[ht]
	\centerline{\includegraphics[width={#1}\textwidth]{#2}}\label{#3}
	\end{figure}}
\newcommand{\figcap}[4]{
	\begin{figure}[ht]
	\centerline{\includegraphics[width={#1}\textwidth]{#2}}
	\caption{{#3}}\label{#4}
	\end{figure}}

% GREEK LETTERS, ETC.
\let\al\alpha
\let\be\beta
\let\gm\gamma
\let\Gm\Gamma
\let\de\delta
\let\De\Delta
\let\si\sigma
\let\Si\Sigma
\let\om\omega
\let\ka\kappa
\let\la\lambda
\let\La\Lambda
\let\ze\zeta
\let\th\theta
\let\Th\Theta
\let\vth\vartheta
\let\Om\Omega

% Set Notation Number fields
\newcommand{\R}{\ensuremath{\mathbb{R}}} %Reals
\newcommand{\C}{\ensuremath{\mathbb{C}}} %Complex
\newcommand{\Q}{\ensuremath{\mathbb{Q}}} %Rational
\newcommand{\Z}{\ensuremath{\mathbb{Z}}} %Integers
\newcommand{\N}{\ensuremath{\mathbb{N}}} %Naturals

% Parenthesis, Brackets, absolute value
\newcommand{\pa}[1]{\left(#1\right)} % encloses the argument using stretchable parentheses
\newcommand{\brac}[1]{\left[#1\right]} % encloses the argument using stretchable square brackets
%\newcommand{\brace}[1]{\left\{#1\right\}} % encloses the argument with braces
\newcommand{\vbrac}[1]{\left\langle#1\right\rangle} % encloses the argument with langle
\newcommand{\absv}[1]{\left|#1\right|} % encloses the argument using stretchable absolute value bars
\newcommand{\dabsv}[1]{\absv{\absv{#1}}}

% variations of \frac and \sfrac
\newcommand{\pfrac}[2]{\pa{\frac{#1}{#2}}} % enclosed in parentheses
\newcommand{\bfrac}[2]{\brac{\frac{#1}{#2}}} % enclosed in square brackets
\newcommand{\afrac}[2]{\absv{\frac{#1}{#2}}} % enclosed in absolute value
\newcommand{\psfrac}[2]{\pa{\sfrac{#1}{#2}}} % sfrac enclosed in parentheses
\newcommand{\bsfrac}[2]{\brac{\sfrac{#1}{#2}}} % sfrac enclosed in square brackets
\newcommand{\asfrac}[2]{\absv{\sfrac{#1}{#2}}} % sfrac enclosed in absolute value
